New Time-Dependent WFC3/IR Inverse Sensitivities

We present new time-dependent inverse sensitivities for the WFC3/IR channel. These were calculated using the sensitivity change slopes measured by \citet{2024wfc..rept....6M} and photometry of five CALSPEC standards (the white dwarfs GRW+70~5824, GD~153, GD~71, G191B2B, and the G-type star P330E) collected from 2009 to 2023. The new inverse sensitivities account for losses of 1-2\% over 15 years, depending on wavelength, and provide an internal photometric precision better than 0.5\% for all wide--, medium--, and narrow-band filters. An updated version of \texttt{calwf3} (v3.7.2) has been developed for use with a new time-dependent image photometry table (IMPHTTAB) and will be used to update the image header photometric keywords following MAST reprocessing, expected in late-2024. Alternatively, the new inverse sensitivities may be computed by the user for a specific observation date by running \texttt{stsynphot}.

==> figures/delta_zp_ref_2024.tex <==
\begin{figure}[!h]
\centering
\includegraphics[width=1.\linewidth]{figures/delta_zp_ref_2024_fig.eps}
%\vspace{-0.5cm}
\captionsetup{type=table, width=.9\linewidth}
\captionof{figure}{Difference between the zeropoints from the new solution evaluated at the reference epoch (May 2009) and the previous solution (top), and the new solution evaluated 15 years later (June 2024) and the previous solution (bottom). The wide-bands are showed in red, medium-bands in blue and narrow-bands in black. The solid black line indicates a difference of 0. \label{fig:comp_ref_2024}}
\end{figure}

